Optimizing Data-Intensive Computations in Existing Libraries with Split Annotations

Data movement between main memory and the CPU is a major bottleneck in parallel data-intensive applications. In response, researchers have proposed using compilers and intermediate representations (IRs) that apply optimizations such as loop fusion under existing high-level APIs such as NumPy and TensorFlow. Even though these techniques generally do not require changes to user applications, they require intrusive changes to the library itself: often, library developers must rewrite each function using a new IR. In this paper, we propose a new technique called split annotations (SAs) that enables key data movement optimizations over unmodified library functions. SAs only require developers to annotate functions and implement an API that specifies how to partition data in the library. The annotation and API describe how to enable cross-function data pipelining and parallelization, while respecting each function's correctness constraints. We implement a parallel runtime for SAs in a system called Mozart. We show that Mozart can accelerate workloads in libraries such as Intel MKL and Pandas by up to 15x, with no library modifications. Mozart also provides performance gains competitive with solutions that require rewriting libraries, and can sometimes outperform these systems by up to 2x by leveraging existing hand-optimized code.

==> tables/compiler-speedup.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\small
\setlength\tabcolsep{4pt} % default value: 6pt
\begin{tabular}{@{}l|ccc|ccc@{}}
\toprule
\multicolumn{1}{c}{} & \multicolumn{3}{c|}{1 thread}                   & \multicolumn{3}{c}{16 threads}                                        \\
\multicolumn{1}{c}{} & Bohrium        & Numba          & Weld          & Bohrium        & Numba          & \multicolumn{1}{l}{Weld}            \\ \midrule
\textbf{BlSh}        & \na            & \na            & \most{1.61}   & \na            & \na            & \green{0.99}                        \\
\textbf{Haver}       & \green{0.74}   & \green{0.91}   & \most{1.10}   & \green{0.59}   & \green{0.77}   & \most{1.21}                         \\
  \textbf{NBody}     & \green{0.81}   & \most{1.29}     & \green{0.81} & \most{1.48}    & 1.12           & 1.38                                \\
  \textbf{Shalw}     &                &                &               &                &                &                                     \\
  \textbf{DaCln}     & \na            &                & \most{4.41}   & \na            &                & \most{1.29}                         \\
\textbf{Crime}       & \na            &                & \most{5.85}   & \na            &                & \most{5.65}                         \\
\textbf{Movie}       & \na            & \na            &               & \na            & \na            &                                     \\
\textbf{Birth}       & \na            & \na            &               & \na            & \na            &                                     \\ \bottomrule
\end{tabular}
\caption{Average speedup of optimizing compilers over SAs on the Python workloads. An
\na entry indicates that the compiler did not support the workload
  without requiring modifications \emph{to the compiler}. \most{Red values} show
  the highest speedup over SAs in each setting, and \green{green values} show cases
  where SAs outperform the compiler.}
\end{table}

